Audio Description Generation in the Era of LLMs and VLMs: A Review of Transferable Generative AI Technologies

Audio descriptions (ADs) function as acoustic commentaries designed to assist blind persons and persons with visual impairments in accessing digital media content on television and in movies, among other settings. As an accessibility service typically provided by trained AD professionals, the generation of ADs demands significant human effort, making the process both time-consuming and costly. Recent advancements in natural language processing (NLP) and computer vision (CV), particularly in large language models (LLMs) and vision-language models (VLMs), have allowed for getting a step closer to automatic AD generation. This paper reviews the technologies pertinent to AD generation in the era of LLMs and VLMs: we discuss how state-of-the-art NLP and CV technologies can be applied to generate ADs and identify essential research directions for the future.

==> tables/Eval-paper-list.tex <==
\begin{table*}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|lccccc|r}
    \toprule
    Research & Venue & Task & Language & Domain & Method | Dataset \\ 
    \midrule
    \citet{Zhang_2024_CVPR} & CVPR'24 & & & \\
    \citet{wang2024tarsier} & arXiv'24 & & & \\
    \citet{mazur2024same} & Universal Access in the Information Society & & & \\
    \citet{liu2023models} & EMNLP'23 & & & \\
    \citet{sarto2023positive} & CVPR'23 & & & \\
    \citet{cripwell2023document} & EACL'23 & & & \\
    \citet{natalie2023supporting} & CHI'23 & & & \\
    \citet{yang2023pilot} & Frontiers in Communication & & & \\
    \citet{arias2023audio} & Journ. Specialised Translation & & & \\
    \citet{yan2023audio} & Perspectives: Studies in Translation Theory and Practice & & & \\
    \citet{munoz2023multimodal} & Journ. Audiovisual Translation & & & \\
    \citet{leong2023audio} & Review of Disability Studies & & & \\
    \citet{lebron2022bertha} & LREC'22 & & & \\
    \citet{shi2022emscore} & CVPR'22 & & & \\
    \citet{wang2022evaluating} & Translation Spaces & & & \\
    \citet{bausells2022audio} & Journ. Audiovisual Translation & & & \\
    \citet{vercauteren2021evaluating} & Revista Tradumàtica & & & \\
    \citet{lopez2021enhancing} & Journ. Audiovisual Translation & & & \\
    \citet{ning2021audio} & Neurocomputing & & & \\
    \citet{ferziger2020audio} & British Journ. Visual Impairment & & & \\
    \citet{gallego2020defining} & AAAL'20 & & & \\
    \citet{wang2020evaluating} & Journ. Audiovisual Translation & & & \\
    \citet{lopez2018audio} & British Journ. Visual Impairment & & & \\
    \citet{jekat2018reception} & BMC'18 & & & \\
    \citet{walczak2018vocal} & Perspectives: Studies in Translatology & & & \\
    \citet{walczak2017creative} & British Journ. Visual Impairment & & & \\
    \citet{fernandez2016machine} & Journ. Translation and Interpretation & & & \\
    \citet{torne2016machine} & Journ. InTRAlinea & & & \\
    \citet{kleege2015audio} & Disability Studies Quarterly & & & \\
    \citet{fernandez2015cross} & Audiovisual Translation in a Global Context & & & \\
    \citet{orero2012eye} & Monografías de Traducción e Interpretación & & & \\
    \citet{vilaro2012evaluation} & IWAAL'12 & & & \\
    \citet{fryer2013visual} & Inputs-Outputs'13 & & & \\
    \citet{braun2007audio} & Linguistica Antverpiensia & & & \\
    \citet{peli1996evaluating} & Journ. Visual Impairment and Blindness & & & \\
    \bottomrule
    \end{tabular}}
    \caption{A collection of research studies related to AD Evaluation. Acronyms: AI - Artificial Intelligence, PS - Psychology, TS - Translation Science, IT - Inclusive Technology}
    \label{tab:paper-collection}
\end{table*}


==> tables/PE-paper-list.tex <==
\begin{table*}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|lccccr}
    \toprule
    Research & Venue & Task & Language & Model & Method | Dataset  \\ 
    \midrule
    Fischer et al. (2024) & EMNLP'24 & & & \\
    \citet{raheja2024medit} & NAACL'24 & & & \\
    \citet{son2024locate} & arXiv'24 & & & \\
    \citet{shu2024rewritelm} & AAAI'24 & & & \\
    \citet{ki2024guiding} & NAACL'24 & & & \\
    \citet{raheja2023coedit} & EMNLP'23 & & & \\
    \citet{zhang2023non} & EMNLP'23 & & & \\
    \citet{laban2023beyond} & arXiv'23 & & & \\
    \citet{kang2023bigvideo} & ACL'23 & & & \\
    \citet{agrawal2022imitation} & ACL'22 & & & \\
    \citet{kim2022improving} & EMNLP'22 & & & \\
    \citet{mallinson2022edit5} & EMNLP'22 & & & \\
    \citet{malmi2022text} & NAACL'22 & & & \\
    \citet{fomicheva2022mlqe} & LREC'22 & & & \\
    \citet{karakanta2022post} & EAMT'22 & & & \\
    \citet{lai2022exploration} & NAACL'22 & & & \\
    \citet{faltings2021text} & NAACL'21 & & & \\
    \citet{zouhar2021neural} & EMNLP'21 & & & \\
    \citet{tardel2021post} & ASLTRW'21 & & & \\
    \citet{wang2021exploring} & NoDaLiDa'21 & & & \\
    \citet{iso2020fact} & ACL'20 & & & \\
    \citet{kasner2020data} & INLG'20 & & & \\
    \citet{mallinson2020felix} & EMNLP'20 & & & \\
    \citet{pavel2020rescribe} & ACM UIST'20 & & & \\
    \citet{shi2020recurrent} & EMNLP'20 & & & \\
    \citet{chollampatt2020can} & EMNLP'20 & & & \\
    \citet{wan2020incorporating} & WMT'20 & & & \\
    \citet{herbig2020mmpe} & ACL'20 & & & \\
    \citet{pal2020transference} & COLING'20 & & & \\
    \citet{malmi2019encode} & EMNLP'19 & & & \\
    \bottomrule
    \end{tabular}
    }
    \caption{A collection of research studies related to AD Post-Editing.}
    \label{tab:paper-collection}
\end{table*}


==> tables/acronyms.tex <==
\begin{table*}[]
    \centering
    \begin{tabular}{ll}
    NLP  & Natural Language Processing \\
    CV & Computer Vision \\
    ADG   & Audio Description Generation \\
    LLM & Large Language Model \\
    VLM & Vision Language Model \\
    DVC & Dense Video Captioning \\
    HCI & Human-Computer Interaction \\
    BLEU & Bilingual Evaluation Understudy \\
    METEOR & Metric for Evaluation of Translation with Explicit Ordering \\
    ROUGE & Recall-Oriented Understudy of Gisting Evalutation \\
    CIDEr & Consensus-based Image Description Evaluation \\
    WMD & Word Mover's Distance \\
    SPICE & Semantic Propositional Image Captioning Evaluation \\
    TE & Text Editing \\
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table*}
